Simulation of primordial object formation

We have included the chemical rate network responsible for the formation of molecular Hydrogen in the N-body hydrodynamic code, Hydra, in order to study the formation of the first cosmological at redshifts between 10 and 50. We have tested our implementation of the chemical and cooling processes by comparing N-body top hat simulations with theoretical predictions from a semi-analytic model and found them to be in good agreement. We find that post-virialization properties are insensitive to the initial abundance of molecular hydrogen. Our main objective was to determine the minimum mass ($M_{SG}(z)$) of perturbations that could become self gravitating (a prerequisite for star formation), and the redshift at which this occurred. We have developed a robust indicator for detecting the presence of a self-gravitating cloud in our simulations and find that we can do so with a baryonic particle mass-resolution of 40 solar masses. We have performed cosmological simulations of primordial objects and find that the object's mass and redshift at which they become self gravitating agree well with the $M_{SG}(z)$ results from the top hat simulations. Once a critical molecular hydrogen fractional abundance of about 0.0005 has formed in an object, the cooling time drops below the dynamical time at the centre of the cloud and the gas free falls in the dark matter potential wells, becoming self gravitating a dynamical time later.

==> texfigs/profiles.tex <==
\begin{figure}
\epsscale{\figscale}
\plotone{\thisdir/figs/mrho_r.col.epsc}

\caption[Mass and overdensity profiles]{\label{massprofiles}The evolution of
the radial profiles of the mass (positively sloped lines) and overdensity
(negatively sloped lines) for baryonic (solid lines) and dark matter (broken
lines) are shown for the most massive object in a cosmological simulation at
redshifts of 24 and 20.  These profiles correspond to the objects indicated in
figure \ref{M200vsz}. The dark matter overdensity increases with the expansion
of the universe, as does the baryon overdensity for $r \gtrsim 3\mathrm{pc}$. 
At $z=28$ enough {\Ht} has formed that the baryons cool efficiently and free
fall into the dark matter potential well.  At $z=20$, $10^7$ years or
approximately one dynamical time later, the object becomes self gravitating.}

\end{figure}


\begin{figure}
\epsscale{\figscale}
\plotone{\thisdir/figs/T_r.col.epsc}

\caption[Temperature profiles]{\label{tempprofiles}The evolution of the
temperature profile of the baryons in the most massive object in a cosmological
simulation at redshifts of 28, 26, and 20.  These profiles correspond to the
objects indicated in figure \ref{M200vsz}.  The core temperature decreases as
time evolves.  Shock heating causes the peak temperature to increase with time,
and as the shock front moves outward the peak temperature occurs at greater
distances from the centre of the object.}

\end{figure}


